Bounded Invariant Checking for Stateflow

Stateflow models are complex software models, often used as part of industrial safety-critical software solutions designed with Matlab Simulink. Being part of safety-critical solutions, these models require the application of rigorous verification techniques for assuring their correctness. In this paper, we propose a refutation-based formal verification approach for analyzing Stateflow models against invariant properties, based on bounded model checking (BMC). The crux of our technique is: i) a representation of the state space of Stateflow models as a symbolic transition system (STS) over the symbolic configurations of the model, and ii) application of incremental BMC, to generate verification results after each unrolling of the next-state relation of the transition system. To this end, we develop a symbolic structural operational semantics (SSOS) for Stateflow, starting from an existing structural operational semantics (SOS), and show the preservation of invariant properties between the two. We define bounded invariant checking for STS over symbolic configurations as a satisfiability problem. We develop an automated procedure for generating the initial and next-state predicates of the STS, and a prototype implementation of the technique in the form of a tool utilising standard, off-the-shelf satisfiability solvers. Finally, we present preliminary performance results by applying our tool on an illustrative example and two industrial models.

==> eptcsdata.tex <==
\providecommand{\firstpage}{38}
\providecommand{\publicationstatus}{M. Luckcuck and M. Farrell; M. Autili, L. Berardinelli,\\ A. Bucaioni and C. Pompilio (Eds.):\\
Formal Methods for Autonomous Systems and \\
Automated and verifiable Software sYstem DEvelopment \\
EPTCS 371, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.371.3}{10.4204/EPTCS.371.3}}

